Maximizing Miner Revenue in Transaction Fee Mechanism Design

Transaction fee mechanism design is a new decentralized mechanism design problem where users bid for space on the blockchain. Several recent works showed that the transaction fee mechanism design fundamentally departs from classical mechanism design. They then systematically explored the mathematical landscape of this new decentralized mechanism design problem in two settings: in the plain setting where no cryptography is employed, and in a cryptography-assisted setting where the rules of the mechanism are enforced by a multi-party computation protocol. Unfortunately, in both settings, prior works showed that if we want the mechanism to incentivize honest behavior for both users as well as miners (possibly colluding with users), then the miner revenue has to be zero. Although adopting a relaxed, approximate notion of incentive compatibility gets around this zero miner-revenue limitation, the scaling of the miner revenue is nonetheless poor. In this paper, we show that if we make a mildly stronger reasonable-world assumption than prior works, we can circumvent the known limitations on miner revenue, and design auctions that generate optimal miner revenue. We also systematically explore the mathematical landscape of transaction fee mechanism design under the new reasonable-world and demonstrate how such assumptions can alter the feasibility and infeasibility landscape.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

#TARGET=puncture-set.pdf 
TARGET=TFM-close.pdf 
TARGET2=TFM-ccs2023.pdf 

all: $(TARGET)
ccs: $(TARGET2)
#eprint:  $(TARGET2)
 
$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<
#	bibtex $(basename $<)
#	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<


$(TARGET2): $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<) 
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.log *.aux *.bbl *.blg *.out *.bak .*.xtx.cache parsetab.py \#*\# *~


==> acknowledge.tex <==
\section*{Acknowledgments}
This work is in part supported by NSF awards 2212746, 2044679, 1704788, a Packard Fellowship, a generous gift from the late Nikolai Mushegian, a gift from Google, and an ACE center grant from Algorand Foundation. 
% The authors would like to thank the anonymous reviewers for their helpful comments.
% We also thank Matt Weinberg
% for helpful technical discussions regarding how to 
% efficiently instantiate our MPC-assisted mechanisms.

==> generalize_distribution.tex <==
\section{Generalize to Arbitrary Distributions}

We can see from the proof of  Theorem~\ref{thm:group-xor} that the incentive compatibility depends on the fact the probability of a random bid larger than or equal to the median is exactly $1/2$. However, for some distributions, it is not necessarily true that $\Pr[b \geq \m] = 1/2$. For example, for a uniform distribution over $\{0,1,2\}$, the probability that a random bid is larger than or equal to the median $\m=2$ is $1/3$. To take care of this, we generalize the parity-based mechanism by forcing the mechanism to split the bid into two groups, such that the probability that a random bid falls into each group is exactly $\frac{1}{2}$.
\begin{mdframed}
    \begin{center}
    {\bf Generalized Parity-based Mechanism}
    \end{center}
    \paragraph{Parameters:} upper bound $c$ of the colluding users, number of bids $n$, the distribution median $\m$, and the probability $p = \Pr[b < \m]$, $p_m = \Pr[b = \m]$.
    
    \paragraph{Mechanism:}
    \begin{itemize}[leftmargin=5mm,itemsep=1pt]
    \item 
    {\it Confirmation rule.}
    Given a bid vector $\bfb = (b_1,\dots, b_n)$,
    \begin{itemize}
        \item Assign a label for each bid as follows. 
        If $b_i< \m$, label it as ${\sf L}$ (for low); if $b_i > \m$, label it as ${\sf H}$ (for high). If $b_i = \m$, label it as ${\sf L}$ with probability $\frac{\frac{1}{2}-p}{p_m}$.
        \item Parse the bid vector $\bids$ into $\lfloor \frac{n}{c + 1}\rfloor$ groups, where the $k$th group $G_k$ is defined as follows. 
        \[
            G_k = \left\{\begin{matrix}
            (b_{(k-1)\cdot (c +1) + 1},\dots,b_{i\cdot (c +1)+1}), &\text{ if } k = 1,\dots, \lfloor \frac{n}{c + 1}\rfloor - 1;\\
            (b_{(k-1)\cdot (c +1) + 1},\dots,b_n), &\text{ if } k = \lfloor \frac{n}{c + 1}\rfloor.
            \end{matrix}\right.
        \]
    Then, for each group $G_k$, let $t_k$ be the number of bids in $G_k$ that are labeled ${\sf H}$. If $t_k$ is odd, then every bid in $G_k$ labeled ${\sf H}$ is confirmed and every bid in $G_k$ labeled ${\sf L}$ is unconfirmed.
    Otherwise, $t_k$ is even, all bids in $G_k$ are unconfirmed.
    \end{itemize}
    \item 
    {\it Payment rule.} All confirmed bids pays $\m$.
    \item 
    {\it Miner revenue rule.}
    For each group $G_k$ with odd $t_k$, miner gets $\m$. 
    Otherwise, for each group $G_k$ with even $t_k$ $\m$ is even, the miner gets nothing from $G_k$.
    \end{itemize}
\end{mdframed}
\begin{theorem}
\label{thm:group-xor}
%Suppose $\bfb$ contains at least one bid from honest users, and the identities of users are known a priori. 
Suppose that each user's true value is independently drawn from a distribution $\mcal{D}$ with median $\m$.
The parity-based mechanism in the Bayesian setting is exact-Bayesian UIC, exact-Bayesian MIC and exact-Bayesian SCP against miners with total mining power $\rho$ in the close system.
\end{theorem}
\begin{proof}
Note that by the definition of median, $p = \Pr[b < \m] \leq \frac{1}{2}$.
Therefore, the probability that a random bid $b$ drawn from $\mcal{D}$ is labeled as ${\sf L}$ is
\begin{align*}
    \Pr[b \text{ labeled }{\sf L}] =& \Pr[b < \m] + \Pr[b \text{ labeled }{\sf L} \mid b = \m]\Pr[b = \m]\\
    =& p + \frac{\frac{1}{2} - p}{p_m}\cdot p_m = \frac{1}{2}.
\end{align*}
Thus, a random bid drawn from the distribution $\mcal{D}$ is labeled ${\sf L}$ (or ${\sf H}$) with probability exactly half. The rest of the proof are same to the proof of Theorem~\ref{thm:group-xor}, where a random bid is smaller than (or larger than and equal to) the median is exactly half.


% Since the identities of users are known a-priori, the miner and users cannot inject any fake bid.
% Moreover, the miner is not allowed to choose which bids are included.
% Thus, we only need to argue exact-UIC and exact-$c$-SCP.
% Since when $\widetilde{n}$ does not exist, nobody is confirmed and miner gets 0, we will only focus on the case where $\widetilde{n}$ exists.

% Note that if $b_i$ is drawn from the distribution $\mcal{D}$, then $x_i$ is a uniform distribution over $\{0,1,\dots,\widetilde{n}-1\}$. Too see this, for any $x\in\{0,\dots,\widetilde{n}-1\}$,
% \[\Pr[x_i = x] = \Pr[x_i = x \mid b_i\geq \m]\Pr[b_i\geq \m]+\Pr[x_i = x \mid b_i < \m]\Pr[b_i < \m] = \frac{1}{\widetilde{n}}.\]
% Now we argue the exact-UIC and exact-$c$-SCP separately.
% \paragraph{Exact-UIC.}
% It suffices to show that user $i$'s utility cannot increase if user $i$ overbids or underbids for any $i$.
% For each group $k$, since $x_j$ for $j\neq i$ are uniformly distributed over $\{0,\dots,\widetilde{n}-1\}$, the sum of $x_j$ in group $G_k$ module $\widetilde{n}$ is also uniformly distributed over $\{0,\dots,\widetilde{n}-1\}$. Thus, 
% \[\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{user $i$ bid }b_i] = p.\]
% Now let $k^*$ denote the group of user $i$.
% Note that user $i$'s bid $b_i$ will be confirmed only if $b_i \geq \m$, and user $i$ needs to pay $\m$ if $b_i$ is confirmed.
% Thus, if $b_i< \m$, user $i$'s utility is $0$. 
% On the other hand, user $i$'s expected utility when bidding $b_i\geq \m$ is
% \[(v_i - \m)\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{user $i$ bid }b_i] = p(v_i - \m).\]
% Therefore, the expected utility of user $i$ when bidding $b_i$ is
% \begin{equation*}
%     \begin{cases}
%     0, & b_i < \m;\\
%     p(v_i-\m), & b_i \geq \m.
%     \end{cases}
% \end{equation*}
% If user $i$'s true value $v_i < \m$, its utility cannot exceed zero, which is the honest case.
% If user $i$'s true value $v_i\geq \m$, its expected utility is at most $(1-p)(v_i - \m)$, which is the expected utility when bidding honestly.
% % Now, suppose user $i$'s true value $v_i \geq \m$.
% % If $b_i$ is confirmed, user $i$'s utility is $v_i - m \geq 0$.
% % Observe that the confirmation of $b_i$ only depends on how many bids are $\geq m$ in the group, so user $i$'s expected utility is the same as long as $b_i \geq m$, which is the same as bidding truthfully.
% % However, if $b_i < m$, it must be unconfirmed, and user $i$'s utility must be zero.
% To sum up, strategic bidding cannot increase user $i$'s utility.

% \paragraph{Exact-$c$-SCP.}
% Since we assume the identities of users are known a-priori,
% a coalition of a miner and up to c user(s) can only deviate from the honest behavior by bidding untruthfully.
% Let $\bids$ denote the bid vector of all users and $\bids_S$ denote the set of bids submitted from the coalition.
% Since each group contains at least $c+1$ bids, there must be at least one bid that comes from the honest user in each group. Equivalently, there is at least one $x_j$ that is drawn uniformly from $\{0,\dots,\widetilde{n}-1\}$ in each group.
% Thus, for all $k$, we have $\Pr[t_k\geq \widetilde{n}(1-p)] = p$ given that the coalition bids $\bids_S$.
% Because the miner revenue of each group is calculated independently, and the revenue of each group $G_k$ only depends on $t_k$, the expected miner-revenue when the coalition bidding $\bids_S$ is
% \begin{align*}
%     \E[\mu(\bids)\mid \text{coalition bids }\bids_S] = \sum_{k\in\lfloor\frac{n}{c+1}\rfloor} \m\cdot\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{coalition bids }\bids_S]=p\cdot \m\cdot\lfloor\frac{n}{c+1}\rfloor,
% \end{align*}
% which will not change no matter how the coalition deviates from the mechanism.
% For each user in the coalition, by the same argument for exact UIC, we conclude that each colluding user's utility cannot increase by bidding untruthfully.
% Therefore, the any deviation from the honest behavior cannot increase the utility of any member in the coalition, so does the joint utility.
% Thus, the mechanism is exact-$c$-SCP.
\end{proof}




==> infinite_ub.tex <==

\input{strict.tex}
% \subsection{Feasibility for Approximate IC: Threshold Posted Price Auction}
% \label{sec:thresholdPosted}

% Without loss of generality, we assume that each user's bid is drawn i.i.d.~from a known distribution $\mathcal{D}$ with the median $\m$ such that $\Pr_{x\sim\mathcal{D}}[x\geq \m] = 1/2$.
% \ke{move this section to appendix}

% \begin{mdframed}
%     \begin{center}
%     {\bf MPC-assisted, threshold-based mechanism}
%     \end{center}
%     \vspace{2pt}
%     \noindent\textbf{Parameters:} lower bound $h$ on the number of honest users, the distribution median $\m$.
%     \vspace{2pt}
%     \textbf{Mechanism:}
%     \begin{itemize}[leftmargin=5mm,itemsep=1pt]
%     \item 
%     {\it Confirmation rule.}
%     Given a bid vector $\bfb = (b_1, \ldots, b_{\ell})$, 
%     for each bid $b_i$, confirm $b_i$ if $b_i \geq \m$.
%     \item 
%     {\it Payment rule.}
%     Each confirmed bid pays $\m$.
%     \item 
%     {\it Miner revenue rule.}
%     Let $s$ be the number of confirmed bids. If $s\geq \frac{h}{4}$, miner gets $\frac{h}{4}\cdot \m$. Otherwise, the miner gets nothing.
%     \end{itemize}
% \end{mdframed}

\begin{theorem}
\label{thm:general-approx-posted-price}
Fix any $h\geq 1$.
The MPC-assisted, threshold-based mechanism is Bayesian UIC, $\epsilon$-MIC, and $\epsilon$-SCP in an $(h,*,*,*)$-environment, where $\eps = \frac{h}{4}\cdot \m \cdot e^{-\frac{h}{8}}$.
\end{theorem}

% \begin{proof}
% First, UIC is easy to prove. 
% Observe that the allocation rule is monotone, and the payment rule is the unique one that satisfies Myerson's Lemma.
% Therefore, the mechanism satisfies UIC.

% \paragraph{$\eps$-MIC.} 
% Recall that the only strategy that a strategic miner can apply is injecting some fake bids.
% Because injecting fake bids smaller than $\m$ does not influence the miner's utility,
% we only consider injecting bids at least $\m$.
% Let $X$ denote the random variable representing the number of honest bids at least $\m$. 
% The only situation where the miner can increase its expected gain by injecting fake bids is $X<\frac{h}{4}$.
% By Chernoff Bound, \ke{add in prelim} we have
% \[\Pr\left[X < \frac{h}{4}\right]\leq e^{-\frac{h}{8}}.\]
% Therefore, the colluding miner can gain at most $\frac{h}{4}\cdot \m\cdot e^{-\frac{h}{8}}$ more expected utility by injecting fake bids.

% \paragraph{$\epsilon$-SCP.} 
% Since the confirmation and the payment of each bid is independent of other bids, and the mechanism is strict Bayesian UIC, the coalition cannot increase colluding users' utilities.
% Therefore, by deviating from the mechanism, the coalition can only try to increase the expected miner revenue. 
% By a similar argument as MIC, the coalition can only increase the expected miner revenue when $X < \frac{h}{4}$, which happens with a probability no more than $e^{-\frac{h}{8}}$.
% It follows that no matter how the coalition deviates, the expected miner's revenue can increase by at most $\rho\cdot \frac{h}{4}\cdot \m \cdot e^{-\frac{h}{8}}$.
% \end{proof}
% The above theorem implies that when the estimate $h$ of the lower bound of the number of honest players is large enough, any coalition can only increase its joint utility by a negligible amount.







==> matrix-fig.tex <==
\section{Matrices in Proof of Claim \ref{clm:infty-norm}}
\label{sec:matrix-fig}

\begin{figure*}
    \centering
    \begin{tikzpicture}
    \draw (0,0) node [scale = 1] {
    \begingroup
    \renewcommand*{\arraystretch}{1.5}
    $\begin{pmatrix}
            \prod_{i=1}^{d}(\bico-z-d+i)\prod_{i=d+1}^{2d}(z+i) & \prod_{i=1}^{d+1}(\bico-z-d-1+i)\prod_{i=d+2}^{2d}(z+i)& \dots & \prod_{i=1}^{2d}(\bico-z-2d+i)\\
            \prod_{i=1}^{d-1}(\bico-z-d+1+i)\prod_{i=d}^{2d}(z+i) & \prod_{i=1}^{d}(\bico-z-d+i)\prod_{i=d+1}^{2d}(z+i) & \dots & \prod_{i=1}^{2d-1}(\bico-z-d+1+i)(z+2d)\\
            \vdots & \vdots & \ddots & \vdots \\
            \prod_{i=1}^{2d}(z+i) & (\bico-z)\prod_{i=2}^{2d}(z+i) &  \dots &  \prod_{i=1}^{d}(\bico-z-d+i)\prod_{i=d+1}^{2d}(z+i)
        \end{pmatrix}.$
        \endgroup
        };
\end{tikzpicture}
    \caption{Matrix form of $B(z)$ in the proof of \cref{clm:infty-norm}.}
    \label{fig:matrix-B}
\end{figure*}

\begin{figure*}
    \centering
    \begin{tikzpicture}
    \draw (0,0) node [scale = 1] {
    \begingroup
    \renewcommand*{\arraystretch}{1.5}
    $\begin{pmatrix}
            \prod_{i=1}^{d}i\cdot \prod_{i=d+1}^{2d}(z+i) & 0& \dots & 0\\
            \prod_{i=1}^{d-1}(i+1)\cdot \prod_{i=d}^{2d}(z+i) & \prod_{i=1}^{d}i\cdot \prod_{i=d+1}^{2d}(z+i) & \dots & 0\\
            \vdots & \vdots & \ddots & \vdots \\
            \prod_{i=1}^{2d}(z+i) & d\cdot \prod_{i=2}^{2d}(z+i) &  \dots &  \prod_{i=1}^{d}i\cdot \prod_{i=d+1}^{2d}(z+i)
        \end{pmatrix}.$
        \endgroup
        };
\end{tikzpicture}
    \caption{Matrix form of $B(\bico-d)$ in the proof of \cref{clm:infty-norm}.}
    \label{fig:triangle-matrix}
\end{figure*}


\begin{figure*}
    \centering
    \begin{tikzpicture}
    \draw (0,0) node [scale = 1]{
    \begingroup
    \renewcommand*{\arraystretch}{1.8}
     $\begin{pmatrix}
            \frac{(\bico-z^*-d+1)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+d)} & \frac{(\bico-z^*-d)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+d+1)}& \dots & \frac{(\bico-z^*-2d+1)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+2d)}\\
            \frac{(\bico-z^*-d+2)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+d-1)} & \frac{(\bico-z^*-d+1)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+d)} & \dots & \frac{(\bico-z^*-2d+2)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+2d-1)}\\
            \vdots & \vdots & \ddots & \vdots \\
            1 & \frac{\bico-z^*}{z^*+1} &  \dots & \frac{(\bico-z^*-d+1)\dots(\bico-z^*)}{(z^*+1)\dots(z^*+d)}
        \end{pmatrix}.$
    \endgroup
    };
\end{tikzpicture}
    \caption{Matrix form of $A'$ in the proof of \cref{clm:infty-norm}.}
    \label{fig:matrix-A}
\end{figure*}


==> oldintro.tex <==
\section{Old Intro}
\subsection{Our Results and Contributions}
%First, consider strict incentive compatibility.
\ignore{Although the 0 miner-revenue 
limitation holds both in the plain model~\cite{foundation-tfm}
and the MPC-assisted model~\cite{crypto-tfm} (and even for Bayesian 
notions of incentive compatibility), 
after examining the two proofs by Chung and Shi~\cite{foundation-tfm}
and Shi et al.~\cite{crypto-tfm} respectively,
we observe an interesting subtlety: {\it the 0 miner-revenue limitation actually holds 
in a stronger sense in the plain model than the MPC-assisted model} --- we will
elaborate on this point later.
Based on this observation, 
}
Our hope is to consider 
a {\it mildly stronger ``reasonable-world''
type assumption} than Shi et al.~\cite{crypto-tfm}, thus allowing us 
circumvent the 0 miner-revenue limitation in the MPC-assisted model (for strict incentive
compatibility).
\ignore{
As we later discuss in \elaine{refer}, 
although the 
0 miner-revenue
limitation holds both in the plain model~\cite{foundation-tfm}
and the MPC-assisted model~\cite{crypto-tfm}, a more careful
examination of 
the two proofs~\cite{foundation-tfm,crypto-tfm}
reveal an interesting subtlety:  
}
More specifically, the mechanisms proposed
by Shi et al.~\cite{crypto-tfm}
{\it implicitly} assume the following reasonable-world assumption:
the strategic coalition 
controls 
no more than $\rho$ fraction of the miners, and no more than $c$ 
users\footnote{Shi et al.~\cite{crypto-tfm} referred to this as achieving 
MIC against any $\rho$-sized miner coalition, achieving SCP
against any $(\rho, c)$-sized miner-user coalition.}.
We will consider a mildly stronger reasonable world which  
promises the following: 
\begin{enumerate}[leftmargin=5mm,itemsep=1pt]
\item 
Just like Shi et al.~\cite{crypto-tfm}, we assume that 
the strategic coalition
controls
no more than $\rho$ fraction of the miners, 
and no more than $c$ users;
\item 
We additionally assume that there is an a-priori known lower bound
$h$ on the number of honest users; naturally, $h$ is also a lower bound on the number of honest bids;
\item 
We additionally assume that 
the number of bids submitted by 
the strategic coalition is  
no more than some a-priori known parameter $d \geq c$.
In other words, here we are assuming while identities
or pseudonyms may be cheap, they are not completely cost-free;
and this is why the strategic coalition cannot  
make up arbitrarily many fake identities 
and submit arbitrarily many fake bids.
\end{enumerate}

\paragraph{New reasonable-world: $(h, \rho, c, d)$-environment.}
Henceforth, 
if the above  
reasonable-world assumptions are promised to hold, we say that 
it is an $(h, \rho, c, d)$-environment,
where $h \geq 1$, $\rho \in (0, 1)$, $c \geq 1$,
and $d \geq c$ 
are a-priori known parameters.
In this paper, we want to design mechanisms 
that satisfy UIC, MIC, and SCP in an $(h, \rho, c, d)$-environment,
while maximizing miner revenue.
%In other words, the mechanism are given the parameters
%$h, \rho, c$ and $d$ as input.

In comparison, the mechanisms in the prior work of  
Shi et al.~\cite{crypto-tfm} receive 
only the a-priori parameters $\rho$
and $c$ as input, and there is no promise about $h$ and $d$, i.e.,  
the resulting mechanisms must work for any choice of $h$ and $d$.
Henceforth, we say that such mechanisms are {\it universal}
in the parameters $h$ and $d$, and that they  
satisfy UIC, MIC, and SCP in an {\it $(*, \rho, c, *)$-environment},
where each $*$ denotes a universal parameter.

An interesting observation 
is that the new strengthened reasonable world
does not help us overcome the 0 miner-revenue limitation
in the {\it plain} model. 
By contrast, our extra assumptions 
indeed invalidate the proof 
of the 0 miner-revenue limitation 
in the {\it MPC-assisted} model.
In other words, 
{\it the 0 miner-revenue limitation actually holds 
in a stronger sense in the plain model~\cite{foundation-tfm} than 
the MPC-assisted model~\cite{crypto-tfm}}.
In the plain model, the limitation holds 
even when 1) the only strategic play is to bid untruthfully, 
i.e., 
a strategic user (possibly colluding with the miner) 
never injects bids or drops out, and a strategic miner 
always implements the rules of the TFM honestly,  
%i.e., the only possible strategic
%play is to bid untruthfully, 
and 2) the mechanism is promised that there are $n-1$ honest bids
for some fixed $n > 2$, and only one strategic bid.  
By contrast, in the MPC-assisted model, 
the proof of the 0 miner-revenue
limitation (for Bayesian incentive compatibility)~\cite{crypto-tfm}
%holds in a weaker sense, since its proof~\cite{crypto-tfm} 
critically depends on 
1) a strategic user's ability
to inject fake bids or drop out; and 2) the fact 
that the TFM must nonetheless provide (Bayesian) UIC, MIC, and SCP  
even when the world consists of only a single strategic user  
(possibly colluding with some miners), and no honest user at all.

Inspired by the above key insights, 
we prove several new results 
that jointly give a complete characterization 
of the miner revenue in $(h, \rho, c, d)$-environments.
Throughout the paper, we assume that in the MPC-assisted model, the total
miner revenue is divided equally among the miners.
%We use two parameters $\rho$ and $c$ to characterize the side-contract-proofness
%of the mechanism, where $\rho \in [0, 1)$ denotes the maximum fraction of miners
%and $c$ denotes the 
%maximum number of users controlled by the strategic coalition.
Since we focus on Bayesian notions of equilibrium, we make the standard assumption  
that each honest user's bid is independently sampled from some a-priori known
distribution $\mcal{D}$. Throughout, we assume that $\mcal{D}$ has bounded support.

%\paragraph{Infinite block size: asymptotic optimality in 
%miner revenue in the known-$h$ model.}
\paragraph{A complete characterization for the infinite block setting.}
This setting is relevant 
because real-world blockchains like Ethereum  
use the recent past to adjust the reserve price, such that 
the vast majority of the time, 
the block size 
can accommodate all users who are willing to pay the reserve price, thus
emulating an ``infinite block size'' scenario.

We show that 
assuming that block size is infinite
and that $c \leq d \leq \frac18 \sqrt{\frac{h}{2\log h}}$,
\elaine{is this correct?}
one can indeed construct a TFM that 
guarantees Bayesian UIC, MIC, and SCP 
in an $(h, \rho, c, d)$-environment, 
and meanwhile achieves 
$\Theta(h)$ miner revenue in expectation (taken
over 
the randomness of the mechanism as well as the honest users' bids).
Importantly, we achieve {\it scalability} in miner revenue 
in the sense that 
when we scale up the bid distribution 
$\mcal{D}$ by a factor of $\alpha$, the miner revenue scales up by $\alpha$ too. 
We also show that $\Theta(h)$ miner revenue 
is asymptotically 
optimal for an $(h, \rho, c, d)$-environment
even for an arbitrarily small $\rho \in (0, 1)$, 
and even for $c = d = 1$. \elaine{is this true}
In particular, we cannot
hope for asymptotically more than 
$\Theta(h)$ expected miner revenue 
even when the actual number of honest users 
far exceeds the anticipated lower bound $h$.

\ignore{
and achieves $\Theta(h \cdot C_{\mcal{D}})$ revenue in expectation (taken
over 
the randomness of the mechanism as well as the honest users' bids), 
where $C_{\mcal{D}}$ 
denotes \elaine{FILL}.
\elaine{what is the assumption we make about D?}
Observe that the miner revenue scales up proportionally with the magnitude
of the distribution $\mcal{D}$.
We also show for any bounded distribution $\mcal{D}$ whose maximum
value is $M$, 
$\Theta(h \cdot M)$
expected miner revenue is the best one can hope for in 
the known-$h$ model. Therefore, our mechanism 
achieves miner revenue that is asymptotically optimal in $h$,
and for natural distributions where 
$C_{\mcal{D}}$ is 
}

More formally, we prove the following theorems
that give tightly matching upper and lower bounds on miner revenue
for the infinite block setting.

\begin{theorem}[Achieving $\Theta(h)$ miner revenue model under
infinite block size]
Suppose that the block size is infinite and that $c \leq d \leq \frac18\sqrt{\frac{h}{2\log h}}$.
For any $h \geq 1$, $d\geq c \geq 1$, and $\rho \in (0, 1)$, 
there exists an MPC-assisted TFM  
that guarantees 
Bayesian UIC, MIC, and SCP 
in an $(h, \rho, c, d)$-environment, 
and meanwhile the mechanism 
achieves $\Theta(h \cdot M_{\mcal{D}})$
expected miner revenue, and  
at least $\Theta(\widetilde{h} \cdot C_{\mcal{D}})$
expected social welfare for the users
where $\widetilde{h} \geq h$ is the 
actual number of honest users
that show up, $M_{\mcal{D}}$
denotes the median of the bid distribution $\mcal{D}$,
and $C_{\mcal{D}} = \E_{x \sim \mcal{D}}[x-M_{\mcal{D}}| x\geq M_{\mcal{D}}]$
is another constant related to the distribution $\mcal{D}$.
\label{thm:intro-inf-opt}
\end{theorem}

\begin{theorem}[$\Theta(h)$ miner revenue is optimal in $(h, \rho, c, d)$-environments]
Fix any 
$h \geq 1$, $d\geq c \geq 1$, and $\rho \in (0, 1)$.
No MPC-assisted TFM 
that simultaneously satisfies 
Bayesian UIC, MIC, and SCP 
in an $(h, \rho, c, d)$-environment
can achieve more than $h \cdot \E(\mcal{D})$
expected miner revenue where $\E(\mcal{D})$
denotes the expectation of the bid distribution $\mcal{D}$. Further,
this limitation on miner revenue holds no matter whether the block
size is finite or infinite.
%, and even for $c = 1$ and for an arbitrarily 
%small positive $\rho$.
\label{thm:intro-h-opt}
\elaine{remark the median later}
\end{theorem}


\paragraph{A complete characterization for the finite block setting.}
In  \Cref{thm:intro-inf-opt}, we focus on the infinite block setting.
An interesting question is whether we can 
get non-trivial results for the finite block setting too. 
\ignore{
The most straightforward
idea is to run the same mechanism
of \Cref{thm:intro-inf-opt} while randomly down-select
to fit in the block size. 
The resulting mechanism indeed 
achieves ex post UIC, Bayesian MIC, and Bayesian SCP,  \elaine{is this true?}
but only for $c = 1$, as stated
in the follow theorem.
}
We show how to modify the  
mechanism of \Cref{thm:intro-inf-opt}
to work in the finite block setting, leading to the following theorem.

\begin{theorem}[Finite block, $c = 1$]
Suppose that the block size is $k$. 
%and fix $c = 1$ and
%any $\rho \in [0, 1)$.
Fix $c = 1$, 
any $h \geq 1$, any $\rho \in (0, 1)$, and any $d$ such
that $c\leq d \leq \frac18 \sqrt{\frac{h}{2\log h}}$.
Then, 
there exists an MPC-assisted TFM %in the known-$h$ model
that satisfies ex post UIC, Bayesian MIC, and  Bayesian SCP \elaine{is this true?} 
in an $(h, \rho, c, d)$-environment;
and  moreover,
the mechanism achieves
$\Theta(\min(h, k) \cdot M_{\mcal{D}})$ expected miner revenue
and 
at least $\Theta(\min(\widetilde{h}, k) \cdot C_{\mcal{D}})$ 
expected social welfare for the users,
where $\widetilde{h}$, $M_{\mcal{D}}$, and $C_{\mcal{D}}$ defined in the same
way as \Cref{thm:intro-inf-opt}.
\elaine{remark the median later}
\label{thm:intro-finite-c1}
\end{theorem}

For $c \geq 2$, it turns out that the answer is more subtle.  
The challenge for $c \geq 2$ is that one user with a small true value
and simply drop out to increase its friend's chances, and  
thus the aforementioned random down-selection idea would fail.
On one hand, we show that there indeed exist 
some bid distributions $\mcal{D}$ such that 
for any choice of $d \geq c \geq 2$ and $\rho \in [0, 1)$, 
using a slight modification of the mechanism 
of  \Cref{thm:intro-inf-opt}, we can get 
$\Theta(h)$ expected miner revenue, while satisfying 
(Bayesian) UIC, MIC, and SCP %for $(\rho, c)$-sized coalitions. 
in an $(h, \rho, c, d)$-environment.
Unfortunately, 
the resulting mechanism appears to degenerate 
in some respects in the sense 
that the social welfare for all users is $0$.
We prove that this is no accident: in fact, 
for any $d \geq c  \geq 2$ and $\rho \in (0, 1)$, 
any MPC-assisted
TFM that simultaneously satisfies
Bayesian UIC, MIC, and SCP must suffer from $0$ total user social welfare
when more than $h$ users show up whose bids are sampled from $\mcal{D}$: 
%when there are actually more than $h$ honest bids, 

\begin{theorem}[Finite block, $c \geq 2$: limit on social welfare]
Suppose that the block size is finite, and fix any $h \geq 1$, any $d \geq c \geq 2$,
and any $\rho \in (0, 1)$.
Then, 
any MPC-assisted TFM 
that simultaneously satisfies 
Bayesian UIC and SCP 
in an $(h, \rho, c, d)$-environment
must suffer from $0$ social welfare 
for the users 
under a bid vector $\bfb\sim \mcal{D}^\ell$
where $\ell > h$.
%when there actually are more than $h$ honest bids.
\label{thm:intro-limit-finite-block}
\end{theorem}

Due to the $0$ social welfare limitation for 
strict incentive compatibility,   
it makes sense to consider approximate incentive compatibility 
for finite blocks and $c \geq 2$.
In this case, we show a feasibility result
with asymptotic optimality in both miner revenue and social welfare,
as stated below:

\begin{theorem}[Approximately incentive compatible mechanism 
for the finite block setting]
%\elaine{FILL}
Fix any $h\geq 1$, $c\geq 1$, and $\rho\in(0,1)$.
Suppose the block size is $k$, 
and let %$\epsilon\geq 2\rho \cdot M_{\mcal{D}}
%\cdot \frac{h}{4}\cdot e^{-\frac{h}{8}}$.
$\epsilon \geq M_{\mathcal{D}}\cdot \frac{h}{2}\cdot e^{-\frac{h}{16}}$. 
% \elaine{FILL}
There is an MPC-assisted TFM that satisfies 
ex post UIC, Bayesian $\epsilon$-MIC, and Bayesian $\epsilon$-SCP 
\elaine{is this correct?}
in $(h, \rho, c, *)$-environments. 
Moreover, 
for sufficiently large $h$, 
the mechanism achieves 
$\Theta(k \cdot M_{\mcal{D}})$
expected miner revenue, 
and $\Theta(k \cdot C_{\mcal{D}})$
expected total user social welfare, 
where $M_{\mcal{D}}$ and $C_{\mcal{D}}$ are defined in the same
way as \Cref{thm:intro-inf-opt}.
%against $(\rho,c)$-sized miner-user coalition for 
%$\epsilon\geq 2\rho \cdot \m \cdot \frac{h}{4}\cdot e^{-\frac{h}{8}}$.
%\end{theorem}
\label{thm:intro-finite-approx}
\end{theorem}



\ignore{
\paragraph{A stronger separation from universal mechanisms.}
Recall that Shi et al.~\cite{crypto-tfm} proved  0 miner-revenue
limitation for any TFM
that satisfies strict UIC, MIC, and SCP in $(*, \rho, c, d)$-environments, i.e.,
mechanisms that are universal in the parameter $h$. 
Their 0 miner-revenue limitation, 
in combination
with our \Cref{thm:intro-inf-opt}, already shows a separation 
between universal and non-universal mechanisms.  
However, Shi et al. did not give a complete characterization
of the miner revenue 
for {\it approximate} incentive compatibility in the universal model.

We prove that even when allowing approximate incentive compatibility, 
any universal, MPC-assisted mechanism
that simultaneously satisfies Bayesian UIC, MIC, and SCP  
must suffer from %\elaine{FILL} 
    at most 
$\frac{8n}{\rho}\left[\frac{\epsilon}{c} + \sqrt{\frac{\E[\mathcal{D}]\epsilon}{c}}\right]$
miner revenue.

%\begin{theorem}[Limit on miner revenue for approximately incentive compatible, universal
%mechanisms]
%\elaine{FILL}
%\label{thm:intro-limit-universal}
%\end{theorem}

\begin{theorem}[Limit on miner revenue for universal mechanism]
\label{thm:intro-limit-universal}
Fix any $d\geq c\geq 1$ and $\rho\in(0,1)$.
Suppose there are $n$ users whose true values are drawn i.i.d. from some distribution $\mcal{D}$.
Given any (possibly randomized) MPC-assisted TFM in an $(*,\rho,c,d)$-environment that is Bayesian $\eps_m$-MIC and Bayesian $\eps_s$-SCP,
it must be that
\begin{equation}
\underset{\bids\sim\mcal{D}^{n}}{\E} [\mu(\bids)]\leq 
    \frac{8n}{\rho}\left[\frac{\epsilon}{c} + \sqrt{\frac{\E[\mathcal{D}]\epsilon}{c}}\right]
\label{eqn:minerrevlimit}
\end{equation}
where $\eps = \eps_s + \eps_m$ and $\mu(\bfb)$ denotes the total miner revenue
under the bid vector $\bfb$.
\end{theorem}
\Cref{thm:intro-limit-universal} says that for any MPC-assisted mechanism that is universal in the
parameter $h$,
the miner revenue must 
{\it scale poorly w.r.t. the magnitude of the bid distribution $\mcal{D}$}.
A special case is when $\epsilon =0$ --- in this case, the above 
theorem says that the miner revenue must be $0$ 
for any universal mechanism (even for Bayesian notions of equilibrium).
%which agrees with what Shi et al. proved~\cite{crypto-tfm}.  

In comparison, the mechanism of \Cref{thm:intro-inf-opt}
enjoys miner revenue that scales proportionally w.r.t. to the magnitude
of the distribution $\mcal{D}$, and moreover, it works even for strict incentive compatibility.
%Since our mechanism in \Cref{thm:intro-inf-opt}
%works for strict incentive compatibility, 
Therefore, the combination of 
\Cref{thm:intro-limit-universal} 
and \Cref{thm:intro-inf-opt}
show an even stronger separation
between the universal and non-universal mechanisms.
Note that Shi et al.~\cite{crypto-tfm} actually proved the special case of 
\Cref{thm:intro-limit-universal} 
for when $c = 1$, but their proof does not readily extend
to the case of general $c$.
}



%\paragraph{Technical highlights.}
%\elaine{to write after roadmap}



\ignore{
\subsection{Our Results and Contributions}


For strict incentive compatibility, although the 0 miner-revenue 
limitation holds both in the plain model 
and the MPC-assisted model (and even for Bayesian 
notions of incentive compatibility), 
after examining the two proofs by Chung and Shi~\cite{foundation-tfm}
and Shi et al.~\cite{crypto-tfm} respectively,
we observe an interesting subtlety. In fact, {\it the 0 miner-revenue limitation holds 
in a stronger sense in the plain model than the MPC-assisted model}.
In the plain model, the limitation holds 
even when 1)  
the only strategic play is to bid untruthfully, 
i.e., 
a strategic user (possibly colluding with the miner) 
never injects bids or drops out, and a strategic miner 
always implements the rules of the TFM honestly,  
%i.e., the only possible strategic
%play is to bid untruthfully, 
and 2) the mechanism is promised that there are $n-1$ honest bids
for some fixed $n > 2$, and only one strategic bid.  
By contrast, in the MPC-assisted model, 
the proof of the 0 miner-revenue
limitation (for Bayesian incentive compatibility)~\cite{crypto-tfm}
%holds in a weaker sense, since its proof~\cite{crypto-tfm} 
critically depends on 
1) a strategic user's ability
to inject fake bids or drop out; and 2) the fact 
that the TFM must nonetheless provide (Bayesian) UIC, MIC, and SCP  
even when the world consists of only a single strategic user  
(possibly colluding with some miners), and no honest user at all.

\elaine{TODO: maybe talk about the permissionless
challenge upfront in the paper}

Inspired by this subtlety, our hope is to overcome
the 0 miner-revenue limitation in the MPC-assisted model  
by introducing a mild 
``reasonable-world type''
assumption: suppose that 
the mechanism is given an {\it a-priori known lower bound
$h$ on the number of honest users.}
Under this mild assumption, we explore whether we can achieve asymptotical
optimality in miner revenue. 
Observe that the known-$h$ assumption does nothing 
in the plain model, %in overcoming the 0 miner-revenue limitation, 
but
it indeed invalidates the proof of the 0 miner-revenue limitation 
in the MPC-assisted model, and for Bayesian notions of incentive compatibility.


We prove several new results 
that jointly give a complete characterization of the known-$h$ model. 
Throughout the paper, we assume that in the MPC-assisted model, the total
miner revenue is divided equally among the miners.
We use two parameters $\rho$ and $c$ to characterize the side-contract-proofness
of the mechanism, where $\rho \in [0, 1)$ denotes the maximum fraction of miners
and $c$ denotes the 
maximum number of users controlled by the strategic coalition.
Since we focus on Bayesian notions of equilibrium, we make the standard assumption  
that each honest user's bid is independently sampled from some a-priori known
distribution $\mcal{D}$.
\ignore{
We make a  
mild assumption on the distribution 
$\mcal{D}$, that is, suppose that the distribution 
has a median (i.e., $1/2$-quantile) and a $3/4$-quantile, where
the $\beta$-quantile $q$ is defined  
as 
the value $q$ such that 
$\Pr_{x \sim \mcal{D}}[x \geq q] = \beta$\footnote{It is easy
to modify the mechanism to work with other quantiles.} 
}


%\paragraph{Infinite block size: asymptotic optimality in 
%miner revenue in the known-$h$ model.}
\paragraph{A complete characterization for the infinite block setting.}
This setting 
is relevant 
because real-world blockchains like Ethereum  
use the recent past to adjust the reserve price, such that 
the vast majority of the time, 
the block size 
exceeds the number of users who are willing to pay the reserve price, thus
emulating an ``infinite block size'' scenario.

We show that given a promise of at least $h$
honest users, and assuming that block size is infinite,  
one can indeed construct a TFM that 
guarantees Bayesian Bayesian UIC, MIC, and SCP 
for any $\rho \in [0, 1)$ and any $c \geq 1$
and meanwhile achieves 
$\Theta(h)$ miner revenue in expectation (taken
over 
the randomness of the mechanism as well as the honest users' bids).
Importantly, we achieve {\it scalability} in miner revenue 
in the sense that 
%the miner revenue scales up
%by a factor of $\alpha$ 
when we scale up the bid distribution 
$\mcal{D}$ by a factor of $\alpha$, the miner revenue scales up by $\alpha$ too. 
We also show that $\Theta(h)$ miner revenue 
is asymptotically 
optimal in the known-$h$ model. In particular, we cannot
hope for asymptotically more than 
$\Theta(h)$ expected miner revenue 
even when the actual number of honest users 
far exceeds the anticipated lower bound $h$.

\ignore{
and achieves $\Theta(h \cdot C_{\mcal{D}})$ revenue in expectation (taken
over 
the randomness of the mechanism as well as the honest users' bids), 
where $C_{\mcal{D}}$ 
denotes \elaine{FILL}.
\elaine{what is the assumption we make about D?}
Observe that the miner revenue scales up proportionally with the magnitude
of the distribution $\mcal{D}$.
We also show for any bounded distribution $\mcal{D}$ whose maximum
value is $M$, 
$\Theta(h \cdot M)$
expected miner revenue is the best one can hope for in 
the known-$h$ model. Therefore, our mechanism 
achieves miner revenue that is asymptotically optimal in $h$,
and for natural distributions where 
$C_{\mcal{D}}$ is 
}

More formally, we prove the following theorems
that give tightly matching upper and lower bounds on miner revenue
in the known-$h$ model.

\begin{theorem}[Achieving $\Theta(h)$ miner revenue model under
infinite block size]
Suppose that the block size is infinite.
%and that the distribution $\mcal{D}$ has a median denoted ${\sf med}(\mcal{D})$
%such that $\Pr_{x \sim \mcal{D}}[x \geq {\sf med}(\mcal{D})] = 1/2$.
There exists an MPC-assisted TFM  
in the known-$h$ model that guarantees 
Bayesian UIC, MIC, and SCP for any $c \geq 1$ and $\rho \in [0, 1)$, 
and meanwhile the mechanism 
achieves
$\Theta(h \cdot {\sf med}(\mcal{D}))$
expected miner revenue, and  
at least $\Theta(\widetilde{h} \cdot {\sf med}(\mcal{D}))$
expected social welfare for the users
where $\widetilde{h} \geq h$ is the 
actual number of honest users
that show up
%\footnote{It is possible to modify
%the mechanism to use a different quantile rather than the median.}.
%\elaine{fix the median}
where ${\sf med}(\mcal{D})$
denotes the median of the bid distribution $\mcal{D}$.
\label{thm:intro-inf-opt}
\end{theorem}

Besides achieving asymptotic optimality 
in miner revenue, the mechanism of \Cref{thm:intro-inf-opt} also 
achieves asymptotical optimality in social welfare for the users
as stated above.
%As mentioned, the mechanism in \Cref{thm:intro-inf-opt} 
%works in the infinite block size setting.  

\begin{theorem}[$\Theta(h)$ miner revenue is optimal in the known-$h$ model]
%Fix any $c \geq 1$ and $\rho \in (0, 1)$.
No MPC-assisted TFM 
in the known-$h$ model that simultaneously satisfies 
Bayesian UIC, MIC, and SCP 
can achieve more than $h \cdot \E(\mcal{D})$
expected miner revenue where $\E(\mcal{D})$
denotes the expectation of the bid distribution $\mcal{D}$. Further,
this limitation on miner revenue holds no matter whether the block
size is finite or infinite, and even for $c = 1$ and for an arbitrarily 
small positive $\rho$.
\elaine{remark the median later}
\end{theorem}

%\paragraph{$0$ social-welfare limitation for the finite block setting.}
\paragraph{A complete characterization for the finite block setting.}
In  \Cref{thm:intro-inf-opt}, we focus on the infinite block setting.
An interesting question is whether we can 
get non-trivial results for the finite block setting too. 
The most straightforward
idea is to run the same mechanism
of \Cref{thm:intro-inf-opt} while randomly down-select
to fit in the block size. 
The resulting mechanism indeed 
achieves Bayesian UIC, MIC, and SCP, but only for $c = 1$, as stated
in the follow theorem.

\begin{theorem}[Finite block, $c = 1$]
Suppose that the block size is $k$, and fix $c = 1$ and
any $\rho \in [0, 1)$.
Then, 
there exists an MPC-assisted TFM in the known-$h$ model
that satisfies Bayesian UIC, MIC, and SCP for $(\rho, c)$-sized coalitions,
and  moreover,
the mechanism achieves
$\Theta(\min(h, k) \cdot {\sf med}(\mcal{D}))$ expected miner revenue
and 
at least $\Theta(\min(\widetilde{h}, k) \cdot {\sf med}(\mcal{D}))$ 
expected social welfare for the users,
where $\widetilde{h}$ is defined in the same
way as \Cref{thm:intro-inf-opt}.
\elaine{remark the median later}
\label{thm:intro-finite-c1}
\end{theorem}

For $c \geq 2$, it turns out that the answer is more subtle.  
The challenge for $c \geq 2$ is that one user with small true value
and simply drop out to increase its friend's chances, and  
thus the aforementioned random down-selection idea would fail.
We show that 
indeed, there exist 
some bid distributions $\mcal{D}$ such that 
for any 
choice of $c \geq 2$ and $\rho \in [0, 1)$, 
using a slight modification of the mechanism 
of  \Cref{thm:intro-inf-opt}, we can get 
$\Theta(h)$ expected miner revenue, while satisfying 
Bayesian UIC, MIC, and SCP for $(\rho, c)$-sized coalitions. 
Unfortunately, 
the resulting mechanism appears degenerate 
in some respects in the sense 
that the social welfare for all users is $0$.
We prove that this is no accident: in fact, 
for any $c \geq 2$ and $\rho \in (0, 1)$, 
any MPC-assisted
TFM that simultaneously satisfies
Bayesian UIC, MIC,
and SCP must suffer from $0$ social welfare for the users when there are more than $h$ bids, 
as stated
in the following theorem: 

\begin{theorem}[Finite block, $c \geq 2$: limit on social welfare]
%\elaine{FILL}
Suppose that the block size is finite, and fix any $c \geq 2$
and $\rho \in (0, 1)$.
Then, 
any MPC-assisted TFM 
in the known-$h$ model that simultaneously satisfies 
Bayesian UIC, MIC, and SCP 
must suffer from $0$ social welfare for the users when the number of bids is
strictly greater than $h$.
%\elaine{for what c and what rho?}
%can achieve more than $h \cdot \E(\mcal{D})$
%expected miner revenue where $\E(\mcal{D})$
%denotes the expectation of the bid distribution $\mcal{D}$. Further,
%this limitation on miner revenue holds no matter whether the block
%size is finite or infinite.
\label{thm:intro-limit-finite-block}
\end{theorem}

Due to the $0$ social-welfare limitation for 
strict incentive compatibility,   
it makes sense to consider approximate incentive compatibility 
for the finite block setting and $c \geq 2$.
In this case, we show a feasibility result
with asymptotic optimality in both miner revenue and social welfare,
as stated in the theorem below:

\begin{theorem}[Approximately incentive compatible mechanism 
for the finite block setting]
\elaine{FILL}
\label{thm:intro-finite-approx}
\end{theorem}



\paragraph{A stronger separation between the known-$h$
and the universal models.}
To differentiate, %from our new known-$h$ model,
henceforth we use the term ``universal model'' to refer
to the model of Shi et al.~\cite{crypto-tfm} 
where the TFM does not know an a-priori lower bound on $h$,
since mechanisms in this model work universally no matter how many honest users
there are.
As mentioned, Shi et al. proved a 0 miner-revenue
limitation for universal mechanisms which, in combination
with our \Cref{thm:intro-inf-opt}, already
shows a separation of the two models for strict incentive compatibility.
However, Shi et al. did not give a complete characterization
of the miner revenue 
for approximate incentive compatibility in the universal model.
We prove that even when allowing approximate incentive compatibility, 
any universal, MPC-assisted mechanism
that simultaneously satisfies Bayesian UIC, MIC, and SCP  
must suffer from \elaine{FILL} miner revenue.

\begin{theorem}[Limit on miner revenue for approximately incentive compatible, universal
mechanisms]
\elaine{FILL}
\label{thm:intro-limit-universal}
\end{theorem}

Since our mechanism in \Cref{thm:intro-inf-opt}
works for strict incentive compatibility, 
\Cref{thm:intro-limit-universal} shows an even stronger separation
between the known-$h$ model and the universal model.
Note that Shi et al.~\cite{crypto-tfm}
actually proved the special case of 
\Cref{thm:intro-limit-universal} 
for when $c = 1$, but their proof does not readily extend
to the case of general $c$.



\paragraph{Additional results.}
Interestingly, we show that all of our feasibility results, namely, 
\Cref{thm:intro-inf-opt}, \Cref{thm:intro-finite-c1}, 
and \Cref{thm:intro-finite-approx}, critically rely on the Bayesian
notion of equilibrium.
As argued by Shi et al.~\cite{crypto-tfm}, the Bayesian notion of equilibrium 
is suitable for the MPC-assisted model since the users
cannot observe others' bids before submitting 
their own.
Had we insisted on an {\it ex post} notion of equilibrium in the MPC-assisted model,
the known-$h$ assumption would not help us overcome the 
impossibility results pertaining to universal mechanisms.
Specifically, 
even in the known-$h$ model, 
any MPC-assisted mechanism that simultaneously achieves ex post UIC 
and SCP must suffer from $0$ miner revenue even for $c = 1$
and an arbitrarily small positive $\rho$.
More generally, 
for approximate but ex post notions of  incentive compatibility, 
even the known-$h$ model is 
subject to the same miner 
revenue limit stated in \Cref{thm:intro-limit-universal}.
Further, the above restrictions on miner revenue hold
no matter whether the block size is finite or infinite.


\paragraph{Technical highlights.}
\elaine{to write after roadmap}





\ignore{
we refine the question  
and ask the following:
\begin{itemize}[leftmargin=6mm]
\item[]
In the MPC-assisted model, 
can we design a TFM that achieves asymptotically optimal miner revenue
assuming some {\it a-priori known   
lower bound $h$ on the number of honest users}?
\end{itemize}
}

}









==> prelim.tex <==
\section{Additional Preliminaries: Ex Post Incentive Compatibility}
\label{sec:expost-ic-defn}
\begin{definition}[Ex post incentive compatibility]
We say that a TFM satisfies ex post 
$\epsilon$-UIC, 
$\epsilon$-MIC, 
and $\epsilon$-SCP 
respectively, for a coalition or individual $\mcal{C}$, 
iff the following conditions hold, respectively:
\begin{itemize}[leftmargin=5mm]
\item 
{\it User incentive compatibility (UIC).}
We say that an MPC-assisted TFM satisfies
ex post $\epsilon$-UIC in some environment $\mcal{E}$, iff 
for any $n$, for any user $i \in [n]$, 
for any bid vector ${\bf b}_{-i}$ 
denoting the bids of everyone else besides $i$, 
for any true value $v_i \in \R^{\geq 0}$
of user $i$, 
for any strategic bid vector ${\bf b}_i$
from user $i$ which could be empty or consist of multiple bids, 
the following holds as long as the conditions required by the environment $\mcal{E}$ are respected:
\[
%\underset{{\bf b}_{-i}\sim \mcal{D}_{-i}}{\E}
{\sf util}^i({\bf b}_{-i}, v_i) \geq
%\underset{{\bf b}_{-i}\sim \mcal{D}_{-i}}{\E} 
%\E_{{\bf b}_{-i} \sim \mcal{D}^{n-1}}
{\sf util}^i({\bf b}_{-i}, {\bf b}_i)
- \epsilon
\]
where ${\sf util}^i({\bf b})$ denotes the expected utility (taken over
the random coins of the TFM)
of user $i$ when the bid vector is ${\bf b}$.
\item 
{\it Miner incentive compatibility (MIC).}
We say that an MPC-assisted TFM satisfies
ex post $\epsilon$-MIC in some environment $\mcal{E}$, iff 
for any miner coalition $\mcal{C}$, 
for any bid vector ${\bf b}_{-\mcal{C}}$, 
for any strategic bid vector ${\bf b}'$ injected
by the miner, 
the following holds as long as the conditions required by the environment $\mcal{E}$ are respected:
\[
%\underset{{\bf b_{-\mcal{C}}\sim \mcal{D}_{-\mcal{C}}}}{\E}
{\sf util}^{\mcal{C}}({\bf b}_{-\mcal{C}}) \geq
%\E_{{\bf b}_{-\mcal{C}} \sim \mcal{D}^{|-\mcal{C}|}}
%\underset{{\bf b_{-\mcal{C}}\sim \mcal{D}_{-\mcal{C}}}}{\E}
{\sf util}^{\mcal{C}}({\bf b}_{-\mcal{C}}, {\bf b}') 
- \epsilon
\]
where ${\sf util}^{\mcal{C}}({\bf b})$
denotes the expected utility (taken over the random coins
of the TFM) of the coalition $\mcal{C}$ when the input bid
vector is ${\bf b}$.
\item 
{\it Side-contract-proofness (SCP).}
We say that an MPC-assisted TFM satisfies
ex post $\epsilon$-SCP in some environment $\mcal{E}$, iff 
for any miner-user coalition, %consisting of at most $\rho$
%fraction of the miners and at most $c$ users, 
for any bid vector $b_{-\mcal{C}}$ submitted by non-coalition-members,
for any true value vector ${\bf v}_{\mcal{C}}$ 
of users in $\mcal{C}$, 
for any strategic bid vector ${\bf b}_{\mcal{C}}$ 
of the coalition 
(whose length may not be equal to the number of users in $\mcal{C}$),
the following holds as long as the requirements of the environment $\mcal{E}$ 
are respected:
\[
%\underset{{\bf b_{-\mcal{C}}\sim \mcal{D}_{-\mcal{C}}}}{\E}
{\sf util}^{\mcal{C}}({\bf b}_{-\mcal{C}}, {\bf v}_{\mcal{C}})\geq
%\E_{{\bf b}_{-\mcal{C}} \sim \mcal{D}^{|-\mcal{C}|}}
%\underset{{\bf b_{-\mcal{C}}\sim \mcal{D}^{-\mcal{C}}}}{\E}
{\sf util}^{\mcal{C}}({\bf b}_{-\mcal{C}}, {\bf b}_{\mcal{C}}) 
- \epsilon
\]
\end{itemize}
\end{definition}
Henceforth, if a mechanism satisfies ex post $\epsilon$-UIC
%(or $\epsilon$-MIC, $\epsilon$-SCP) respectively 
for $\epsilon = 0$ (i.e., the {\it strict} incentive compatibility case), 
we often omit writing the $\epsilon$,
and simply say that the mechanism satisfies 
ex post UIC. 
The terms ``ex post MIC'', ``ex post SCP'' are similarly defined.

Recall that in the game representing the plain model, strategic players can choose their actions 
{\it after} having observed the bids submitted by honest users.  
This gives rise to the following fact which essentially says it does not make sense
to consider Bayesian notions of equilibrium in the plain model.

\begin{fact}
Any plain-model TFM that satisfies 
\emph{Bayesian} $\epsilon$-UIC (or \emph{Bayesian} $\epsilon$-MIC, \emph{Bayesian} $\epsilon$-SCP resp.)
in some environment $\mcal{E}$
must also satisfy 
\emph{ex post} $\epsilon$-UIC (or \emph{ex post} $\epsilon$-MIC, \emph{ex post} $\epsilon$-SCP resp.).
\label{fct:plainexpost}
\end{fact}


% \subsection{Probability Tools}
% \begin{lemma}[Chernoff bound, Corollary A.1.14~\cite{alon2016probabilistic}]
% \label{lem:chernoff}
% Let $X_1$,$\dots$, $X_n$ be independent Bernoulli random variables. Let $\mu = \E\left[\sum_{i=1}^n X_i\right]$. Then, for any $\epsilon\in(0,1)$, it holds that
% \[\Pr\left[\sum_{i=1}^n X_i \leq (1-\epsilon)\mu\right]\leq e^{-{\epsilon^2}\mu/2}.\]
% \end{lemma}



==> revenue-bound-h.tex <==
%\section{Bounds on Miner Revenue}

%In this section, we extend the bounds on the miner revenue in \cite{crypto-tfm} to the known-$h$ model.
\ignore{
In \cref{section:strict-IC-known-h}, we prove bounds on the total miner revenue 
in the known-$h$ setting.
In \cref{section:revenue-bound-honest-majority}, we show that even if in the MPC-assisted model, and we assume that at least half of the bids come from honest users, the miner revenue is bounded by $\underset{\bids\sim\mcal{D}}{\E} [\bids]$, where $\mcal{D}$ is the distribution of users' true values.
That is, although many users submit their bids to the mechanism, the miner can at most get the revenue from \emph{one} user.
}



==> xor-based-mechanism.tex <==
\section{Exact Incentive Compatibility under Bayesian Setting}


\subsection{Prelim: Myerson's Lemma under Bayesian Setting}
In this section, we introduce the Myerson's Lemma in the Bayesian Setting.
Recall that in the Bayesian setting, when each user decides its strategy, it only knows its true value, while other players' true values are drawn from a known distribution.

Recall that $\bids_{-i}$ denotes all but user $i$'s bid, and $(\bids_{-i}, b_i) = \bids$.
We also let $\mcal{D}_{-i}$ to denote $\mcal{D}_1\times\dots\times\mcal{D}_{i-1}\times\mcal{D}_{i+1}\times\dots\times\mcal{D}_n$, which denotes the distribution of other users' true values. 
\ke{Do we need to emphasize here that this result only uses bidding unfaithfully?}

\begin{lemma}[Myerson's Lemma~\cite{}]
Let $\mcal{D} = \mcal{D}_1\times\dots\times\mcal{D}_n$ be the joint distribution of users' true values.
Let $({\bf x}, {\bf p}, \mu)$ be a single-parameter TFM that is exact-UIC.
Then, it must be that  
\begin{enumerate}[leftmargin=5mm]
	\item 
	The allocation rule ${\bf x}$ is {\it monotonically non-decreasing}.
	% where monotone is defined as follows.
	% Consider ${\bf b} := (b_1, \ldots, b_m)$, and let ${\bf b}_{-i}$ be
	% the vector obtained when we remove $b_i$ from ${\bf b}$.
	% An allocation rule ${\bf x}$ is said to be monotone
	% iff for any ${\bf b} := (b_1, \ldots, b_m)$, 
	Formally, for any user $i$, and any $b'_i > b_i$, 
	it must be that $\EXPT_{\bfb_{-i}\sim \otherdist} \left[x_i({\bf b}_{-i}, b'_i)\right]  \geq \EXPT_{\bfb_{-i}\sim \otherdist} \left[x_i({\bf b}_{-i}, b_i)\right] $.
	\item 
	The payment rule ${\bf p}$ is defined as follows.
	For any user $i$, and bid $b_i$ from user $i$,
	it must be
	\begin{equation}\label{eq:payment}
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[p_i(\bfb_{-i}, b_i)\right] 
		= \EXPT_{\bfb_{-i}\sim \otherdist} \left[b_i \cdot x_i(\bfb_{-i}, b_i) - \int_0^{b_i} x_i(\bfb_{-i}, t) dt\right].
	\end{equation}
	\end{enumerate}
	\label{lem:myerson}
\end{lemma}

\begin{lemma}[Technical lemma implied by the proof of Myerson's Lemma~\cite{myerson,myerson-lecture-hartline}]
	Let $f(z)$ be a non-decreasing function. 
	Suppose that $ z \cdot (f(z')-f(z)) \leq g(z') - g(z) \leq z' \cdot (f(z')-f(z))  $ 
	for any $z' \geq z \geq 0$, and moreover, $g(0) = 0$.
	Then, it must be that 
	\[
	g(z) = z \cdot f(z) - \int_0^{z} f(t) dt.
	\]
	\label{lem:sandwich}
\end{lemma}

\begin{lemma}[Lemma 4.8 in~\cite{foundation-tfm}]
\label{lemma:randomInequality}
    Let $({\bf x}, {\bf p}, \mu)$ be any (possibly randomized) TFM.
	If $({\bf x}, {\bf p}, \mu)$ is 1-SCP against miners with mining power $\rho$, then for any bid vector $\bfb$, user $i$, and $r, r'$ such that $r < r'$, it must be \[
		r \cdot \left(x_i(\bfb_{-i}, r') - x_i(\bfb_{-i},r)\right)
		\leq \pi_{\bfb_{-i}}(r') - \pi_{\bfb_{-i}}(r)
		\leq r' \cdot \left(x_i(\bfb_{-i}, r') - x_i(\bfb_{-i},r)\right),
	\]
where $\pi_{\bfb_{-i}}(r):= p_i(\bfb_{-i},r) - \rho\mu(\bfb_{-i},r)$.
\end{lemma}
\begin{proof}
\ke{proof is same except for adding $\rho$.}
\end{proof}


% \subsection{Parity-based Mechanism}
% \ke{Move it to roadmap, }
% From the Theorem~\ref{thm:impossible-non-decreasing}, we can see that it is impossible to design a mechanism with non-decreasing revenue. 
% Therefore, in this section, we give a mechanism that achieves exact UIC, MIC and $(n-1)$-SCP under the interim setting.
% We assume that every user's true value is drawn \emph{independently} from a known distribution $\mcal{D}$ with midian ${\sf mid}$.
% We first start with a warm up mechanism where the expected miner revenue is $\frac{1}{2}\m$, irrelevant to the number of users. 
% To better convey the idea, we assume that the probability that $\Pr_{b \sim \mathcal{D}}[b > \m] = 1/2$ for now.

% \begin{mdframed}
%     \begin{center}
%     {\bf Parity-based Mechanism}
%     \end{center}
%     \paragraph{Parameters:} the median $\m$ \hao{Discuss whether we want to use the term ``block size'' or more general term for general auction}
    
%     \paragraph{Mechanism:}
%     \begin{itemize}[leftmargin=5mm,itemsep=1pt]
%     \item 
%     {\it Inclusion rule.}
%     \hao{no inclusion rule in MPC setting?}
%     Include all bids in the pool.
%     \item 
%     {\it Confirmation rule.}
%     Given a bid vector $\bfb = (b_1,\dots, b_n)$, let $t$ be the number of bids that are equal to or larger than $\m$.
%     If $t$ is odd, every bid equal to or larger than $\m$ is confirmed.
%     Otherwise if $t$ is even, no bid is confirmed.
%     \item 
%     {\it Payment rule.}
%     Each confirmed bid in the block pays $\m$.
%     \item 
%     {\it Miner revenue rule.}
%     If $t$ is odd, the miner is paid $\m$.
%     \end{itemize}
% \end{mdframed}

% \begin{theorem}
% \label{thm:single-xor}
% Suppose each user's true value is drawn from $\mcal{D}$ with the median $\m$ such that $\Pr_{b \sim \mathcal{D}}[b > \m] = 1/2$. 
% Moreover, at least one bid in the block comes from an honest user.
% Then the parity-based mechanism is exact-UIC, exact-MIC and exact-$c$-SCP for all $c$.
% \end{theorem}
% \begin{proof}
% In the following, we prove the three properties individually.

% \paragraph{Exact-UIC.}
% Fix any user $i$, let $v_i$ denote the true value of user $i$, and $b_i$ denote the bid submitted by user $i$. Note that user $i$ can also inject some fake bids.
% Since we assume at least one bid in the block comes from an honest user, it must be $\Pr[t \text{ is odd}] = \Pr[t \text{ is even}] = \frac{1}{2}$ given user $i$'s bids.
% Because the confirmation of each bid only depends on the parity of $t$ and the payment is always $\m$ if the bid is confirmed, injecting fake bids cannot increase users' utility.
% Thus, it suffices to show that user $i$'s utility cannot increase if user $i$ overbids or underbids.
% Notice that $b_i$ is confirmed only when $b_i \geq \m$, and user $i$ needs to pay $\m$ if $b_i$ is confirmed.
% Moreover, user $i$'s utility is zero if $b_i$ is unconfirmed, and user $i$'s utility is $v_i - \m$ if $b_i$ is confirmed.
% Therefore, the expected utility of user $i$ when bidding $b_i\bf$ is
% \begin{equation*}
%     \begin{cases}
%     0, & b_i < \m;\\
%     \frac{1}{2}(v_i-\m), & b_i \geq \m.
%     \end{cases}
% \end{equation*}
% Thus, if user $i$'s true value $v_i < \m$, its expected utility cannot exceed zero, which is the expected utility when bidding honestly.
% If user $i$'s true value $v_i\geq \m$, its expected utility is at most $\frac{1}{2}(v_i - \m)$, which is the expected utility when bidding honestly.
% % Now, suppose user $i$'s true value $v_i \geq m$.
% % If $b_i$ is confirmed, user $i$'s utility is $v_i - m \geq 0$.
% % Observe that the confirmation of $b_i$ only depends on how many bids are $\geq m$ in the group, so user $i$'s expected utility is the same as long as $b_i \geq m$, which is the same as bidding truthfully.
% % However, if $b_i < m$, it must be unconfirmed, and user $i$'s utility must be zero.
% To sum up, strategic bidding cannot increase user $i$'s utility.
% \ke{Is this $c$-UIC..?}
% \paragraph{Exact-MIC.}
% A miner can only choose to inject fake bids. Note that miner's revenue only depends on the parity of $t$. 
% Let $\bids_S$ be the set of bids inject by the miner.
% Then by the assumption that there is at least one honest bid $b$ drawn from $\mcal{D}$, the probability that $b\geq \m$ is exactly half. 
% Therefore, 
% \[\Pr[t \text{ is odd} \mid \text{miner inject }\bids_S] = \Pr[t \text{ is even}\mid \text{miner inject }\bids_S] = \frac{1}{2}.\]
% Thus, the expected miner utility given $\bids_S$ is that
% \begin{align*}
%     \E[\mu(\bids) \mid \text{miner inject }\bids_S] &= \m \cdot \Pr[t \text{ is odd} \mid \text{miner inject } \bids_S] - \text{payment for }\bids_S\leq \frac{1}{2}\m,
% \end{align*}
% where $\frac{1}{2}\m$ is the expected miner utility when behaving honestly.
% Henceforth, the miner has no incentive to deviate from the mechanism.
% %A miner has two kinds of strategies to deviate from honest behavior: not to include all bids and to inject fake bids. 
% % Without loss of generality, we assume that the miner chooses the included bids first, and then inject some fake bids.
% % Let $\bfb$ be the bid vector that the miner prepares, where $\bfb$ may or may not include all bids and the miner may also inject some fake bids in $\bfb$.
% % Let $t$ be the number of bids in $\bfb$ that are equal to or larger than $m$.
% % Because each bid is drawn from $\mcal{D}$ with the medium $m$, it must be $\Pr[t \text{ is odd}] = \Pr[t \text{ is even}] = \frac{1}{2}$ as long as there is a bid comes from an honest user. 
% % Because the miner's utility only depends on the parity of $t$, not to include all bids and to inject fake bids do not increase the miner's expected utility.
% \ke{the miner has to include all bids?}
% \paragraph{Exact-$c$-SCP.}
% A coalition of a miner and up to c user(s) can perform the mix of the following two strategies: bidding untruthfully and injecting fake bids\footnote{Notice that it does not matter the injecting fake bids come from the miner or the colluding users.}.
% Let $\bfb$ be the bid vector that the mechanism receives, where $\bfb_S$ is the bids submitted from the coalition.
% By the same analysis, the probability that $t$ is odd given that the coalition submit bids $\bids_S$ is exactly $\frac{1}{2}$.
% Because the miner's utility only depends on the parity of $t$, the deviation does not increase the miner's expected utility.
% Moreover, notice that the argument for exact-UIC only assumes at least one bid in $\bfb$ comes from an honest user, by the same argument, we conclude that each colluding user's utility cannot increase by injecting fake bids or bidding untruthfully.
% To sum up, the any deviation from the honest behavior cannot increase the utility of any member in the coalition, so does the joint utility.
% Thus, the mechanism is exact-$c$-SCP for all $c$.
% % A coalition of a miner and up to c user(s) has three kinds of strategies to deviate from
% % the honest behavior: the miner may not inot to include all bids, the miner can inject fake bids,
% % and some of the user(s) can bid untruthfully. 
% % Let $\bfb$ be the bid vector that the miner prepares, where $\bfb$ may or may not include all bids, the coalition may also inject some fake bids in $\bfb$\footnote{Notice that it does not matter the injecting fake bids come from the miner or the colluding users.}, and some colluding users may not bid their true values.
% % Because each bid is drawn from $\mcal{D}$ with the medium $m$, it must be $\Pr[t \text{ is odd}] = \Pr[t \text{ is even}] = \frac{1}{2}$ as long as there is a bid comes from an honest user. 
% % Because the miner's utility only depends on the parity of $t$, the deviatioin does not increase the miner's expected utility.
% % Finally, notice that the argument for exact-UIC only assumes at least one bid in $\bfb$ comes from an honest user, by the same arugment, we conclude that each colluding user's utility cannot increase by injecting fake bids or bidding untruthfully.
% % To sum up, the any deviation from the honest behavior cannot increase the utility of any member in the coalition, so does the joint utility.
% % Thus, the mechanism is exact-$c$-SCP for all $c$.
% \end{proof}


\subsection{Lower Bound in the Open System}
In the open ID system, strategic players can choose to inject fake bids.
The following result shows that if we allow the strategic players to inject fake bids, then the miner's revenue can only be $0$ if the mechanism is UIC, MIC, and $1$-SCP.

We first show that if a TFM is UIC and 1-SCP, then the miner revenue must be independent from each user's bid. Without loss of generality, we assume that $0$ is the minimum value in the support of $\mcal{D}_i$ for $i\in[n]$. 
\begin{lemma}
	\label{lemma:constantRevenue}
	Let $\mcal{D} = \mcal{D}_1\times\dots\times\mcal{D}_n$ be the joint distribution of users' true values.
	Let $({\bf x}, {\bf p}, \mu)$ be any (possibly randomized) TFM.
	If $({\bf x}, {\bf p}, \mu)$ is UIC and 1-SCP against miners with mining power $\rho$, then
	for any user $i$, any bid $b$, it must be 
	\begin{equation}
	\label{eqn:constant-revenue}
	    \EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i}, b)\right]  = \EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i}, 0)\right].
	\end{equation}

	In other words, the miner's revenue is a constant that is independent of user $i$'s bid $b$ when other bids $\bfb_{-i}$ are drawn from the distribution $\otherdist$.
	%\hao{We may want to define $\otherdist = \mcal{D} \times \cdots \times \mcal{D}$.}
\end{lemma}
\begin{proof}
	\hao{This proof is just a minor modification from Lemma 4.8 and Thm 4.7 in \cite{}.}
	For any vector $\bfb_{-i}$, we define $\widetilde{\pi}_{\bfb_{-i}}(r)$ as \[
		\widetilde{\pi}_{\bfb_{-i}}(r) = p_i(\bfb_{-i},r) - \rho\mu(\bfb_{-i},r) - 
		(p_i(\bfb_{-i},0) - \rho\mu(\bfb_{-i},0)).
	\]
	By Lemma~\ref{lemma:randomInequality}, 
	and the fact that definition of $\widetilde{\pi}_{\bfb_{-i}}(r)$
	and ${\pi}_{\bfb_{-i}}(r)$ differs by only a fixed constant,
	it must be that 
	\begin{equation}
			r \cdot \left(x_i(\bfb_{-i}, r') - x_i(\bfb_{-i},r)\right)
			\leq \widetilde{\pi}_{\bfb_{-i}}(r') - \widetilde{\pi}_{\bfb_{-i}}(r)
			\leq r' \cdot \left(x_i(\bfb_{-i}, r') - x_i(\bfb_{-i},r)\right).
	\label{eqn:sandwich}
	\end{equation}
	Because Eq.(\ref{eqn:sandwich}) holds for any $\bfb_{-i}$, we have \[
		r \cdot \left(\EXPT_{\bfb_{-i}\sim \otherdist} \left[x_i(\bfb_{-i}, r')\right] - \EXPT_{\bfb_{-i}\sim \otherdist} \left[x_i(\bfb_{-i},r)\right]\right)
		\leq \EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r')\right] - \EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r)\right],
	\]
	and \[
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r')\right] - \EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r)\right]
		\leq r' \cdot \left(\EXPT_{\bfb_{-i}\sim \otherdist} \left[x_i(\bfb_{-i}, r')\right] -\EXPT_{\bfb_{-i}\sim \otherdist} \left[ x_i(\bfb_{-i},r)\right]\right).
	\]

	Now, observe that the above expression exactly 
	agrees with the ``payment sandwich'' in 
	the proof of Myerson's Lemma~\cite{myerson,myerson-lecture-hartline}\ke{citation}.
	Furthermore, we have that 
	$\EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(0)\right] = 0$
	by definition; and 
	${\bf x}$ must be monotone because the TFM is UIC and satisfies
	Myerson's Lemma. 
	%Recall that the proof of Myerson's Lemma
	%essentially showed that for any quantity 
	%$\widetilde{\pi}_{\bfb_{-i}}(\cdot)$ that satisfies
	%the inequality
	%specified by 
	%Equation~(\ref{eqn:sandwich}), and moreover,
	%$\widetilde{\pi}_{\bfb_{-i}}(0) = 0$ and ${\bf x}$ is monotone,
	%then, 
	Due to Lemma~\ref{lem:sandwich}, 
	it must be that 
	$\EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(\cdot)\right]$ obeys the unique payment rule
	specified by Myerson's Lemma; that is, 
	\[
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r)\right] = 
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[b_i \cdot x_i(\bfb_{-i}, b_i) - \int_0^{b_i} x_i(\bfb_{-i}, t) dt \right].
	\]
	%We therefore conclude that 
	%$\widetilde{\pi}_{\bfb_{-i}}(0)$
	%should satisfy the 
	On the other hand, since the TFM is UIC, its payment rule  
	itself must also satisfy the same expression (Eq.(\ref{eq:payment})), that is, 
	\[
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[p_i(\bfb_{-i}, b_i)\right] 
		= \EXPT_{\bfb_{-i}\sim \otherdist} \left[b_i \cdot x_i(\bfb_{-i}, b_i) - \int_0^{b_i} x_i(\bfb_{-i}, t) dt\right].
	\]
	We therefore have that 
	\[
		\EXPT_{\bfb_{-i}\sim \otherdist} \left[\widetilde{\pi}_{\bfb_{-i}}(r)\right] 
	= \EXPT_{\bfb_{-i}\sim \otherdist} \left[p_i(\bfb_{-i}, b_i)\right].
	\]
	In other words, $\EXPT_{\bfb_{-i}\sim \otherdist} \left[\rho\mu(\bfb_{-i},r)\right] =  \EXPT_{\bfb_{-i}\sim \otherdist} \left[\rho\mu(\bfb_{-i},0)\right] - \EXPT_{\bfb_{-i}\sim \otherdist} \left[p_i(\bfb_{-i},0)\right]$.
	Because $p_i(\bfb_{-i},0) = 0$ for any $\bfb_{-i}$, we conclude $\EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i},r)\right] =  \EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i},0)\right]$.
\end{proof}

\noindent Note that in the proof of Lemma~\ref{lemma:constantRevenue}, we only consider the strategy space of bidding unfaithfully. \ke{elaborate more on this?}
\begin{remark}
A more general form of \eqref{eqn:constant-revenue} is
\[\EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i}, b)\right]  = \EXPT_{\bfb_{-i}\sim \otherdist} \left[\mu(\bfb_{-i}, {\sf min}_i)\right],\]
where ${\sf min}_i$ is the infimum of the support of $\mcal{D}_i$. 
Throughout the paper, we will assume that $0$ is the minimum value in the support of the distributions of users' true values. It can be replaced with $\min\{\supp{\mcal{D}_i}\}$ in a more general form. \ke{move to somewhere ealier?}
%For better presentation in the paper we just assume that ${\sf min}_i = 0$.
\end{remark}

Now we show that, if in addition the mechanism $\mecha$ is MIC in the open system, then the miner revenue can only be $0$.
%\ke{add the condition that at least one honest user}
\begin{theorem}
\label{thm:inject-constantRevenue}
Let $\{\mcal{D}^{(n)}\}_n$ be a sequence of distributions where  $\mcal{D}^{(n)} = \mcal{D}_1\times\dots\times\mcal{D}_{n}$ is the joint distribution of $n$ users' true values, where user $i$'s true value is drawn from $\mcal{D}_i$ independently.
Let $\mecha$ be any randomized TFM. If $\mecha$ is exact-UIC, exact-MIC and 1-SCP against miners with mining power $\rho$, then 
\[\underset{\bids\sim\mcal{D}^{(n)}}{\E} [\mu(\bids)]=0.\]
\end{theorem}
\ke{This thm requires independence.}
\begin{proof}
For any $n\geq 2$, we have the following claim:
\begin{lemma}
\label{lem:inject-induction}
If $\mecha$ is MIC against miners with mining power $\rho$, then $\underset{\bids\sim\mcal{D}^{(n)}}{\E} [\mu(\bids)] \leq \underset{\bids'\sim\mcal{D}^{(n-1)}}{\E} [\mu(\bids')]$.
\end{lemma}
For now assume Lemma~\ref{lem:inject-induction} holds and we explain why Theorem~\ref{thm:inject-constantRevenue} follows from it. The proof of Lemma~\ref{lem:inject-induction} appears right afterwards.
By induction on $n$, we have that 
\[\underset{\bids\sim\mcal{D}^{(n)}}{\E} [\mu(\bids)] \leq \underset{b\sim\mcal{D}_{1}}{\E} [\mu(b)].\]
By Lemma~\ref{lemma:constantRevenue}, for any $b\in\supp{\mcal{D}_1}$, it should be that $\mu(b) = \mu(0)$. Therefore, 
\[\underset{b\sim\mcal{D}_{1}}{\E} [\mu(b)]\leq \mu(0) = 0,\]
where the last equality comes from the requirement that the miner's revenue cannot exceeds the payment of the single identity, who will pay at most what it bids.
% Since for $n=1$, there is only one user whose true value is drawn from $\mcal{D}_1$, we have that $\mu(b)\leq b$ since the miner's revenue should be no more than the user's payment, which is further upper bounded by the user's bid. Therefore, 
% $\underset{b\sim\mcal{D}_{1}}{\E} [\mu(b)]\leq \E[\mcal{D}_1]$.
Theorem~\ref{thm:inject-constantRevenue} thus follows.
\end{proof}

\paragraph{Proof of Lemma~\ref{lem:inject-induction}}
Since $\mecha$ is exact-MIC against mining power $\rho$, it must be that
\begin{equation}
    \underset{\bids\sim\mcal{D}^{(n-1)}}{\E} [\rho \mu(\bids, 0)]\leq \underset{\bids\sim\mcal{D}^{(n-1)}}{\E} [\rho \mu(\bids)].\label{eqn:inject-induction}
\end{equation}

Otherwise, the colluding miners can inject a bid $0$ and increase its miner revenue while it does not need to pay anything for injecting the $0$-bid. This violates the MIC condition.

By the law of total expectation, we have that
\begin{align*}
    \underset{\bids\sim\mcal{D}^{(n)}}{\E} [\mu(\bids)] &= \int_{r\in\supp{\mcal{D}_n}} \underset{\bids'\sim\mcal{D}^{(n-1)}}{\E} [\mu(\bids', r)] f(r) dr & \\
    &=\int_{r\in\supp{\mcal{D}_n}} \underset{\bids'\sim\mcal{D}^{(n-1)}}{\E} [\mu(\bids', 0)] f(r) dr &\text{By Lemma~\ref{lemma:constantRevenue}}\\
    &=\underset{\bids'\sim\mcal{D}^{(n-1)}}{\E} [\mu(\bids', 0)] \leq \underset{\bids'\sim\mcal{D}^{(n-1)}}{\E} [\mu(\bids')] &\text{By \eqref{eqn:inject-induction}}
\end{align*}

\input{non-decreasing}

\subsection{Upper Bound in the Close System}
\label{section:parity-based}
In this section, we introduce a mechanism in the close ID system, that is exact UIC, MIC and 1-SCP against miners with mining power $\rho$ and achieves linear miner-revenue.
\ke{Only when $c$ is a constant. Do we have other lower bounds for $c$ not a constant? like $\Theta(n/c)$?}
Note that $\Theta(n)$ is a trivial upper bound on the miner-revenue, as each user $i$ can pay at most $\max(\supp{\mcal{D}_i})$. 
Therefore our mechanism achieves optimal miner-revenue up to a constant factor.
We assume that each user's bids is drawn i.i.d. from a known distribution $\mathcal{D}$ with median $\m$.
We first start with the simple case like continuous distribution where $\Pr_{b \sim \mathcal{D}}[b \geq \m] = 1/2$.
\begin{mdframed}
    \begin{center}
    {\bf Parity-based Mechanism}
    \end{center}
    \paragraph{Parameters:} upper bound $c$ of the colluding users, the mining power $\rho_j$ of miner $j$ for $j=1,\dots,m$, and the median $\m$ of the distribution $\mcal{D}$.
    
    \paragraph{Mechanism:}
    \hao{We need to mention the mechanism replace $\bot$ with $0$ somewhere.}
    \hao{Corner case: if $n < c$, the mechanism should reject any bid.}
    
    \begin{itemize}[leftmargin=5mm,itemsep=1pt]
    % \item 
    % {\it Inclusion rule.}
    % \hao{no inclusion rule in MPC setting?}
    % Choose the highest $B$ bids into the block.
    \item 
    {\it Confirmation rule.}
    Given a bid vector $\bfb = (b_1,\dots, b_n)$, parse it into $\lfloor \frac{n}{c + 1}\rfloor$ groups, where the $k$th group $G_k$ is defined as follows. 
    \[
    G_k = \left\{\begin{matrix}
        (b_{(k-1)\cdot (c +1) + 1},\dots,b_{i\cdot (c +1)+1}), &\text{ if } k = 1,\dots, \lfloor \frac{n}{c + 1}\rfloor - 1;\\
        (b_{(k-1)\cdot (c +1) + 1},\dots,b_n), &\text{ if } k = \lfloor \frac{n}{c + 1}\rfloor.
    \end{matrix}\right.
    \]
    Then, for each group $G_k$, let $t_k$ be the number of bids in $G_k$ that are equal to or larger than $\m$. If $t_k$ is odd, then every bid in $G_k$ equal to or larger than $\m$ is confirmed and every bid in $G_k$ smaller than $\m$ is unconfirmed.
    Otherwise, $t_k$ is even, all bids in $G_k$ are unconfirmed.
    \item 
    {\it Payment rule.}
    All confirmed bids in the block pay $\m$.
    \item 
    {\it Miner revenue rule.}
    For each group $G_k$ with odd $t_k$, miner $j$ gets $\rho_j \cdot \m$. 
    Otherwise, for each group $G_k$ with even $t_k$, the miner gets nothing from $G_k$.
    \end{itemize}
\end{mdframed}

\begin{remark}
When we pick $c$ to be $0$, the parity-based mechanism just degenerate to posted price auction with reserved price $\m$, which is exact-UIC and exact-MIC in close system. \ke{check this remark}
\end{remark}
%\hao{Remark: when $c = 0$, the mechanism is posted-price with the price $m$.}

\begin{theorem}
\label{thm:group-xor}
%Suppose $\bfb$ contains at least one bid from honest users, and the identities of users are known a priori. 
Suppose that each user's true value is independently drawn from a distribution $\mcal{D}$ with median $\m$ that satisfies $\Pr_{b \sim \mathcal{D}}[b \geq \m] = 1/2$.
The parity-based mechanism is exact-UIC, exact-MIC and exact-$c$-SCP against miners with total mining power $\rho$ in the close system.
%\hao{When users are known a priori and the mechanism is executed by MPC, we have MIC for free. Do we need to write it in the theorem?}
\end{theorem}
\begin{proof}
Because we are considering the close ID system, the miners and users cannot inject any fake bid.
Moreover, the miners are not allowed to choose which bids are included. \ke{this is noly guaranteed in hybrid-world? do we need to add that the mechanism is correctly implemented?}
Thus, we only need to show exact-UIC and exact-$c$-SCP.

\paragraph{Exact-UIC.}
It suffices to show that user $i$'s utility cannot increase if user $i$ overbids or underbids for any $i$.
For any group $k\in\lfloor\frac{n}{c+1}\rfloor$, the probability $\Pr[t_k \text{ is odd}] = \Pr[t_k \text{ is even}] = \frac{1}{2}$ given user $i$'s bid $b_i$.
Now let $k^*$ denote the group of user $i$.
Note that $b_i$ will be confirmed only if $b_i \geq \m$, and user $i$ needs to pay $\m$ if $b_i$ is confirmed.
Moreover, user $i$'s utility is zero if $b_i$ is unconfirmed, and user $i$'s utility is $v_i - \m$ if $b_i$ is confirmed.
Therefore, the expected utility of user $i$ when bidding $b_i$ is
\begin{equation*}
    \begin{cases}
    0, & b_i < \m;\\
    \frac{1}{2}(v_i-\m), & b_i \geq \m.
    \end{cases}
\end{equation*}
Thus, if user $i$'s true value $v_i < \m$, its utility cannot exceed zero, which is the honest case.
If user $i$'s true value $v_i\geq \m$, its expected utility is at most $\frac{1}{2}(v_i - \m)$, which is the expected utility when bidding honestly.
% Now, suppose user $i$'s true value $v_i \geq \m$.
% If $b_i$ is confirmed, user $i$'s utility is $v_i - m \geq 0$.
% Observe that the confirmation of $b_i$ only depends on how many bids are $\geq m$ in the group, so user $i$'s expected utility is the same as long as $b_i \geq m$, which is the same as bidding truthfully.
% However, if $b_i < m$, it must be unconfirmed, and user $i$'s utility must be zero.
To sum up, strategic bidding cannot increase user $i$'s utility.

\paragraph{Exact-$c$-SCP.}
Because we assume the identities of users are known a-priori,
a coalition of a miner and up to c user(s) can only deviate from the honest behavior by bidding untruthfully.
Let $\bids$ denote the bid vector of all users and $\bids_S$ denote the set of bids submitted from the coalition.
%For each group $G_k$, let $t_k$ be the number of bids in $G_k$ that are equal to or larger than $m$.
Since each group contains at least $c+1$ bids, there must be at least one bid comes from the honest user in each group.
Thus, for all $k$, we have $\Pr[t_k \text{ is odd}] = \Pr[t_k \text{ is even}] = \frac{1}{2}$ given that the coalition bids $\bids_S$.
Because the miner revenue of each group is calculated independently, and the revenue of each group $G_k$ only depends on the parity of $t_k$, the expected total miner-revenue when the coalition bidding $\bids_S$ is
\begin{align*}
    \E[\mu(\bids)\mid \text{coalition bids }\bids_S] = \sum_{k\in\lfloor\frac{n}{c+1}\rfloor} \cdot\m\cdot\Pr[t_k \text{ is odd} \mid \text{coalition bids }\bids_S]=\frac{\m}{2}\cdot\lfloor\frac{n}{c+1}\rfloor,
\end{align*}
which will not change no matter how the coalition deviates from the mechanism. Thus the miners in the coalition cannot increase their expected utility be deviating from the mechanism.
For each user in the coalition, by the same argument for exact UIC, we conclude that each colluding user's utility cannot increase by bidding untruthfully.
Therefore, the any deviation from the honest behavior cannot increase the utility of any member in the coalition, so does the joint utility.
Thus, the mechanism is exact-$c$-SCP.
\end{proof}


\subsubsection{Generalizing to Arbitrary Distributions}
We can see from the proof of  Theorem~\ref{thm:group-xor} that the incentive compatibility depends on the fact the the probability of a random bid larger than or equal to the median is exactly $1/2$. However, for some distributions, it is not necessarily true that $\Pr[b \geq \m] = 1/2$. For example, for a uniform distribution over $\{0,1,2\}$, the probability that a random bid is larger than or equal to the median $\m=2$ is $1/3$. To take care of this, we generalize the parity-based mechanism by forcing the mechanism to split the bid into two groups, such that the probability that a random bid falls into each group is exactly $\frac{1}{2}$.
\begin{mdframed}
    \begin{center}
    {\bf Generalized Parity-based Mechanism}
    \end{center}
    \paragraph{Parameters:} upper bound $c$ of the colluding users, number of bids $n$, the distribution median $\m$, and the probability $p = \Pr[b < \m]$, $p_m = \Pr[b = \m]$.
    
    \paragraph{Mechanism:}
    \begin{itemize}[leftmargin=5mm,itemsep=1pt]
    \item 
    {\it Confirmation rule.}
    Given a bid vector $\bfb = (b_1,\dots, b_n)$,
    \begin{itemize}
        \item Assign a label for each bid as follows. 
        If $b_i< \m$, label it as ${\sf L}$ (for low); if $b_i > \m$, label it as ${\sf H}$ (for high). If $b_i = \m$, label it as ${\sf L}$ with probability $\frac{\frac{1}{2}-p}{p_m}$.
        \item Parse the bid vector $\bids$ into $\lfloor \frac{n}{c + 1}\rfloor$ groups, where the $k$th group $G_k$ is defined as follows. 
        \[
            G_k = \left\{\begin{matrix}
            (b_{(k-1)\cdot (c +1) + 1},\dots,b_{i\cdot (c +1)+1}), &\text{ if } k = 1,\dots, \lfloor \frac{n}{c + 1}\rfloor - 1;\\
            (b_{(k-1)\cdot (c +1) + 1},\dots,b_n), &\text{ if } k = \lfloor \frac{n}{c + 1}\rfloor.
            \end{matrix}\right.
        \]
    Then, for each group $G_k$, let $t_k$ be the number of bids in $G_k$ that are labeled ${\sf H}$. If $t_k$ is odd, then every bid in $G_k$ labeled ${\sf H}$ is confirmed and every bid in $G_k$ labeled ${\sf L}$ is unconfirmed.
    Otherwise, $t_k$ is even, all bids in $G_k$ are unconfirmed.
    \end{itemize}
    \item 
    {\it Payment rule.} All confirmed bids pays $\m$.
    \item 
    {\it Miner revenue rule.}
    For each group $G_k$ with odd $t_k$, miner gets $\m$. 
    Otherwise, for each group $G_k$ with even $t_k$ $\m$ is even, the miner gets nothing from $G_k$.
    \end{itemize}
\end{mdframed}
\begin{theorem}
\label{thm:group-xor}
%Suppose $\bfb$ contains at least one bid from honest users, and the identities of users are known a priori. 
Suppose that each user's true value is independently drawn from a distribution $\mcal{D}$ with median $\m$.
The parity-based mechanism is exact-UIC, exact-MIC and exact-$c$-SCP against miners with total mining power $\rho$ in the close system.
\end{theorem}
\begin{proof}
Note that by the definition of median, $p = \Pr[b < \m] \leq \frac{1}{2}$.
Therefore, the probability that a random bid $b$ drawn from $\mcal{D}$ is labeled as ${\sf L}$ is
\begin{align*}
    \Pr[b \text{ labeled }{\sf L}] =& \Pr[b < \m] + \Pr[b \text{ labeled }{\sf L} \mid b = \m]\Pr[b = \m]\\
    =& p + \frac{\frac{1}{2} - p}{p_m}\cdot p_m = \frac{1}{2}.
\end{align*}
Thus, a random bid drawn from the distribution $\mcal{D}$ is labeled ${\sf L}$ (or ${\sf H}$) with probability exactly half. The rest of the proof are same to the proof of Theorem~\ref{thm:group-xor}, where a random bid is smaller than (or larger than and equal to) the median is exactly half.


% Since the identities of users are known a-priori, the miner and users cannot inject any fake bid.
% Moreover, the miner is not allowed to choose which bids are included.
% Thus, we only need to argue exact-UIC and exact-$c$-SCP.
% Since when $\widetilde{n}$ does not exist, nobody is confirmed and miner gets 0, we will only focus on the case where $\widetilde{n}$ exists.

% Note that if $b_i$ is drawn from the distribution $\mcal{D}$, then $x_i$ is a uniform distribution over $\{0,1,\dots,\widetilde{n}-1\}$. Too see this, for any $x\in\{0,\dots,\widetilde{n}-1\}$,
% \[\Pr[x_i = x] = \Pr[x_i = x \mid b_i\geq \m]\Pr[b_i\geq \m]+\Pr[x_i = x \mid b_i < \m]\Pr[b_i < \m] = \frac{1}{\widetilde{n}}.\]
% Now we argue the exact-UIC and exact-$c$-SCP separately.
% \paragraph{Exact-UIC.}
% It suffices to show that user $i$'s utility cannot increase if user $i$ overbids or underbids for any $i$.
% For each group $k$, since $x_j$ for $j\neq i$ are uniformly distributed over $\{0,\dots,\widetilde{n}-1\}$, the sum of $x_j$ in group $G_k$ module $\widetilde{n}$ is also uniformly distributed over $\{0,\dots,\widetilde{n}-1\}$. Thus, 
% \[\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{user $i$ bid }b_i] = p.\]
% Now let $k^*$ denote the group of user $i$.
% Note that user $i$'s bid $b_i$ will be confirmed only if $b_i \geq \m$, and user $i$ needs to pay $\m$ if $b_i$ is confirmed.
% Thus, if $b_i< \m$, user $i$'s utility is $0$. 
% On the other hand, user $i$'s expected utility when bidding $b_i\geq \m$ is
% \[(v_i - \m)\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{user $i$ bid }b_i] = p(v_i - \m).\]
% Therefore, the expected utility of user $i$ when bidding $b_i$ is
% \begin{equation*}
%     \begin{cases}
%     0, & b_i < \m;\\
%     p(v_i-\m), & b_i \geq \m.
%     \end{cases}
% \end{equation*}
% If user $i$'s true value $v_i < \m$, its utility cannot exceed zero, which is the honest case.
% If user $i$'s true value $v_i\geq \m$, its expected utility is at most $(1-p)(v_i - \m)$, which is the expected utility when bidding honestly.
% % Now, suppose user $i$'s true value $v_i \geq \m$.
% % If $b_i$ is confirmed, user $i$'s utility is $v_i - m \geq 0$.
% % Observe that the confirmation of $b_i$ only depends on how many bids are $\geq m$ in the group, so user $i$'s expected utility is the same as long as $b_i \geq m$, which is the same as bidding truthfully.
% % However, if $b_i < m$, it must be unconfirmed, and user $i$'s utility must be zero.
% To sum up, strategic bidding cannot increase user $i$'s utility.

% \paragraph{Exact-$c$-SCP.}
% Since we assume the identities of users are known a-priori,
% a coalition of a miner and up to c user(s) can only deviate from the honest behavior by bidding untruthfully.
% Let $\bids$ denote the bid vector of all users and $\bids_S$ denote the set of bids submitted from the coalition.
% Since each group contains at least $c+1$ bids, there must be at least one bid that comes from the honest user in each group. Equivalently, there is at least one $x_j$ that is drawn uniformly from $\{0,\dots,\widetilde{n}-1\}$ in each group.
% Thus, for all $k$, we have $\Pr[t_k\geq \widetilde{n}(1-p)] = p$ given that the coalition bids $\bids_S$.
% Because the miner revenue of each group is calculated independently, and the revenue of each group $G_k$ only depends on $t_k$, the expected miner-revenue when the coalition bidding $\bids_S$ is
% \begin{align*}
%     \E[\mu(\bids)\mid \text{coalition bids }\bids_S] = \sum_{k\in\lfloor\frac{n}{c+1}\rfloor} \m\cdot\Pr[t_k\geq \widetilde{n}(1-p) \mid \text{coalition bids }\bids_S]=p\cdot \m\cdot\lfloor\frac{n}{c+1}\rfloor,
% \end{align*}
% which will not change no matter how the coalition deviates from the mechanism.
% For each user in the coalition, by the same argument for exact UIC, we conclude that each colluding user's utility cannot increase by bidding untruthfully.
% Therefore, the any deviation from the honest behavior cannot increase the utility of any member in the coalition, so does the joint utility.
% Thus, the mechanism is exact-$c$-SCP.
\end{proof}

% \textcolor{red}{TODO
% \begin{itemize}
%     \item Every user is drawn from different distribution (or even correlated?)
%     \item Can expected miner revenue larger than 0.25 for uniform distribution? Can we prove that it is optimal?
% \end{itemize}
% }

